Graph Integration for Diffusion-Based Manifold Alignment

Data from individual observations can originate from various sources or modalities but are often intrinsically linked. Multimodal data integration can enrich information content compared to single-source data. Manifold alignment is a form of data integration that seeks a shared, underlying low-dimensional representation of multiple data sources that emphasizes similarities between alternative representations of the same entities. Semi-supervised manifold alignment relies on partially known correspondences between domains, either through shared features or through other known associations. In this paper, we introduce two semi-supervised manifold alignment methods. The first method, Shortest Paths on the Union of Domains (SPUD), forms a unified graph structure using known correspondences to establish graph edges. By learning inter-domain geodesic distances, SPUD creates a global, multi-domain structure. The second method, MASH (Manifold Alignment via Stochastic Hopping), learns local geometry within each domain and forms a joint diffusion operator using known correspondences to iteratively learn new inter-domain correspondences through a random-walk approach. Through the diffusion process, MASH forms a coupling matrix that links heterogeneous domains into a unified structure. We compare SPUD and MASH with existing semi-supervised manifold alignment methods and show that they outperform competing methods in aligning true correspondences and cross-domain classification. In addition, we show how these methods can be applied to transfer label information between domains.

==> ideas.tex <==
To select $t$, try using VNE on the normalized off diagonal blocks only;
Try using RF-GAP proximities with the following methods:
    * Using just known correspondances (similar to GDI)
    * Using class proximity averages
    * Using some form of combination

For off-diag blocks (or perhaps the entire joint block matrix) apply PageRank trick.


Prior to taking diffusion steps, the off-diagonal blocks have, on average, much lower values due to missing correspondences. We can try rescaling the main diagonals by $\mu$, and the off diagonals by $\nu$, then rescaling to sum to one after each time step, to give more emphasis on either within-domain similarity or cross-domain similarity.

Need a way to automatically check the mean/median values of kernels (off and main separately) during $t$ update steps. Can you this information to rescale to balance emphasis between withim-class/without-class matching.



For joint embedding, perhaps need to customize the MDS optimization function to give flexibility to have loose/strict matching between known correspondances.

To help with this, we may need to rescale off-diagonal blocks to reset maximum values to 1, do so separately for main diagonal blocks.


Instead of a use for manifold alignment, use the RF-GAP and $\alpha$-decaying kernels as the main diagonal blocks. Learn a single representation of both supervised and unsupervised embeddings by defining all correspondences in the off-diagonal block matrices.

Look at the stationary distribution of the block matrix. How do the densities of the off-diagonal blocks compare with the main diagonals?


Apply density normalization~\cite{lafon2006datafusion} prior to constructing the diffusion operators, maybe also after joining?

The local density \( p(x_i) \) for each point \( x_i \) is estimated using a Gaussian kernel:

\[
p(x_i) = \sum_{j} \exp\left(-\frac{\| x_i - x_j \|^2}{2 \sigma^2}\right)
\]

% Density Normalized Kernel
The kernel \( K \) is adjusted based on the local densities to create a density-normalized kernel \( K_{\text{norm}} \):

\[
K_{\text{norm}}(x_i, x_j) = \frac{K(x_i, x_j)}{\sqrt{p(x_i) \cdot p(x_j)}}
\]

% Row Normalized Kernel
To ensure the resulting matrix is a proper stochastic matrix, the density-normalized kernel \( K_{\text{norm}} \) is row-normalized:

\[
K_{\text{row-norm}}(x_i, x_j) = \frac{K_{\text{norm}}(x_i, x_j)}{\sum_{k} K_{\text{norm}}(x_i, x_k)}
\]


Perhaps used Nystrom method (or geometric harmonics, if it makes sense) to extend to new points. This can also help with the train-test split problem for validation.


Use weighted majority vote for cross-domain labeling. Similar to RF-GAP, but using $W_{XY}$ and/or $W_{YX}$.


Discuss how edge weights are iteratively added; how is our thresholding done? At row-normalized scale, or un-normalized then on scale of original W?


Review the construction of Lafon's construction in~\cite{lafon2006datafusion} on page 7. (Algorithm 3). Perhaps use their way (step 2) to select $t$ and intrinsic dimensionality.

The authors map each domain to a diffusion embedding, where the time steps, $t$, is selected separately for each domain to preserve $k - 1$ eigenvectors. An affine function\footnote{I didn't find explicitly how this function is defined} is defined to map from $\R^{k-1}$ to $\R^{k-1}$, satisfying the landmark constraints.


For known connections, what if we remove the 1 for self-similarity?


Build a repository of datasets specific to the multi-modal / alignment problem. set this up as a benchmark study for multiple alignment models.


Assign non-zero value for unknown correspondence. Perhaps try the median value? Average of medians across each domain?

Can we use the diffusion operator or cross-domain similarities in an optimal transport problem to form a coupling matrix?

==> other_methods.tex <==
Unsupervised:
The authors of~\cite{liu2019mmd-ma} describe an unsupervised manifold alignment method based on maximum mean discrepancy, called MMD-MA. 

and GUMA (generalized unsupervised manifold alignment)~\cite{cui2014guma}, 

==> raw.tex <==

\cite{wang2011manifold}

% ``
% The problem of alignment can be formalized as dimensionality reduction with constraints
% induced by the correspondences among data sets. In many application domains of inter-
% est, data appears high-dimensional, but often lies on low-dimensional structures, such as a
% manifold, which can be discretely approximated by a graph
% ''


% ``
% In other words, manifold alignment discovers a unifying representation of
% all the initially separate datasets that preserves the qualities of each individual dataset and
% highlights the similarities between the datasets. Though this new representation may not
% be the actual "original dataset," if such an entity exists, it should re
% ect the structure that
% the original dataset would have.
% ''

"In this case, if the proteins are actually different, there may be
no ``original dataset" that both observed datasets represent, there may only be a structural
similarity between the two datasets which allows them to be represented in similar locations
in a new coordinate frame."

% ``
% Manifold alignment preserves simi-
% larities within each dataset being aligned and correspondences between the datasets being
% aligned by giving each dataset a new coordinate frame that re
% ects that dataset's underlying
% manifold structure. As such, the main assumption of manifold alignment is that any datasets
% being aligned must lie on the same low dimensional manifold. Furthermore, the algorithm
% requires a similarity function that returns the similarity of any two instances within the same
% dataset with respect to the geodesic distance along that manifold.
% ''

% ``
% In some situations, such as the Europarl example, the required similarity function may
% re
% ect semantic similarity. In this case, the unifying representation discovered by manifold
% alignment represents the semantic space of the input datasets. Instances that are close with
% respect to Euclidean distance in the latent space will be semantically similar, regardless
% of their original dataset. In other situations, such as the protein example, the underlying
% manifold is simply a common structure to the datasets, such as related covariance matrices
% or related local similarity graphs. In this case, the latent space simply represents a new
% coordinate system for all the instances that is consistent with geodesic similarity along the
% manifold.
% ''

See general formulation on pages 8-9 of~\cite{wang2011manifold}

% ``
% In other words, manifold alignment maps each dataset
% to a new joint latent space where locally similar instances within each dataset and given
% corresponding instances across datasets are close or identical in that space
% ''


``
% Second, manifold alignment views each individual dataset as belonging to one larger
% dataset. 
Since all the datasets have the same manifold structure, the graph Laplacians associated with each dataset are all discrete approximations of the same manifold, and
thus, the diagonal concatenation of these Laplacians, along with the off-diagonal matrices
filled with correspondence information, is still an approximation of that manifold.
''

``
Embedding this joint Laplacian combines these ideas. By using a graph embedding al-
gorithm, manifold alignment preserves the local similarities and correspondence information
encoded by the joint Laplacian.
''


``
A corollary of this algorithm is that any embedding technique that depends on the similarities (or distances) between data instances can also find a unifying representation of
disparate datasets. To perform this extension, the embedding algorithm must use both
the regular similarities within each datasets and must treat correspondence information as
an additional set of similarities for instances from different datasets, thus viewing multiple
datasets as all belonging to one joint dataset. Running the embedding algorithm on this
joint dataset results in a unified set of features for the initially disparate datasets.
''

Related fields or algorithms: CCA, graph matching, data fusion, information fusion


\cite{lafon2006datafusion}

``
. First, we show that by carefully normalizing the
Markov matrix, the embedding can be made
invariant to the density of the sampled data points;
thus, solving the problem of data fusion encountered
with other eigenmaps methods.
. Then, we address the problem of out-of-sample
extension and we explain how to adaptively extend
empirical functions to new samples using the geometric harmonics. In particular, this allows us to
extend the diffusion coordinates to new data points.
. Last, we take advantage of the density-invariant
representation of data sets provided by the diffusion
coordinates to derive a simple data matching algorithm based on geometrical embeddings alignment.

''


``By increasing t, one propagates the local or short-term
influence of each node to its nearest neighbors, and this
means that t also plays the role of a scale parameter. The
comparison of these conditional probabilities introduces a
notion of proximity that accounts for the connectivity of the
points in the graph. In particular, unlike the shortest path or
geodesic distance, this metric is robust to noise as it involves
an integration along all paths of length t starting from x or z.
Empirical evidence supporting this claim is provided in [13].
''


``
This means
that most of the variables that describe each data points are
highly correlated, at least locally, or equivalently, that the
data set has a low intrinsic dimensionality. In this case, the
high-dimensional representation of the data is an unfortunate
(but often unavoidable) artifact of the choice of sensors or the
acquisition device. Therefore, it should be possible to obtain
low-dimensional representations of the samples. Note that
since the correlation between variables might only be local,
classical global dimension reduction methods like Principal
Component Analysis and Multidimensional Scaling do not
provide, in general, an efficient dimension reduction.
''

``
More precisely, if the data are assumed to
approximately lie on a manifold, then the eigenmap representation
depends on the density of the points on this
manifold[5].Thisissue is ofcriticalimportancein applications
as one often needs to merge data that were produced by the
same source but acquired with different devices or sensors, at
various sampling rates and possibly on different occasions. In
that case, it is necessary to have a canonical representation of
the data that retains the intrinsic constraints of the samples
(e.g., manifold geometry) regardless of the particular distribution
of the data points sampled by different devices.
''

``
First, we show that by carefully normalizing the
Markov matrix, the embedding can be made
invariant to the density of the sampled data points;
thus, solving the problem of data fusion encountered
with other eigenmaps methods.
''

``
But
rather than giving a list of recipes, we would like to underline
the fact that the choice of the weight function should be entirely
application-driven. The weight function or kernel describes the
first-order interaction between the data points as it defines the
nearest neighbor structures in the graph. It should capture a
notion of similarity as meaningful as possible with respect to
the application and, therefore, could very well take into
account any type of prior knowledge on the data. The analysis
of the data provided by the diffusion techniques depends
heavily on the choice of the weight function.
''

``
In particular, unlike the shortest path or
geodesic distance, this metric is robust to noise as it involves
an integration along all paths of length t starting from x or z.
Empirical evidence supporting this claim is provided in~\cite{lafon2006dm-course-grain}.
''


``
However, working with the
data in its original form can be quite difficult as the two sets
typically consist of measurements of very different nature.
For instance, X1 could be a collection of measurements
related to wether in a given region, whereas X2 could describe
agriculture production in the same region. As a consequence,
it is almost always impossible to directly compare the two
data sets, simply because they might not be represented using
the same type of features. The main idea that we introduce
here is that the diffusion maps provide a canonical
representation of data sets reflecting their intrinsic geometry.
This new representation is based on the graph structure of a
set, that is, the neighbor relationship between points, and not
on their original feature representation. As a consequence,
instead of comparing the data sets in their original forms, it can be
much more efficient to compare their embeddings.
''


``
Ham et al.~\cite{ham2005ssma} align the manifolds,
given a set of a priori corresponding nodes or landmarks. A
constrained formulation of the graph Laplacian based
embeddings is derived by including the given alignment
information. First, they add a term fixing the embedding
coordinates of certain samples to predefined values. Both sets
are then embedded separately, where certain samples in each
set are mapped to the same embedding coordinates. Second,
they describe a dual embedding scheme, where the constrained
embeddings of both sets are computed simultaneously,
and the embeddings of certain points in both data
sets are constrained to be identical.
''


``
The diffusion maps provide a
nonlinear reduction of dimensionality and, therefore, our
scheme is appropriate for the alignment of high-dimensional
data sets with low-intrinsic dimensionality. In addition, as
explained in the previous sections, if we use the density invariant diffusion maps, the alignment scheme will be
insensitive to the different distributions of points of the two
data sets.
''

\cite{lahat2015datafusion-overview}
``
Motivations for data fusion are numerous. They include
obtaining a more unified picture and global view of the system
at hand; improving decision making; exploratory research;
answering specific questions about the system, such as
identifying common versus distinctive elements across modalities
or time; and in general, extracting knowledge from data
for various purposes.
''

``
A key property of multimodality is complementarity, in the sense
that each modality brings to the whole some type of added
value that cannot be deduced or obtained from any of the
other modalities in the setup. In mathematical terms, this
added value is known as diversity.
''

``
Not less important, it serves as a lesson that
fusing modalities can yield undesired results and severe
degradation of performance if the underlying relationships
between modalities are not properly understood.
''

``
In the absence of
additional assumptions, a simulation study favors equal
weight to each data entry regardless of its data set of origin,
over the alternative approach of weighting data sets by the
number of their respective entries [147]. This approach is
generalized to the case of missing values, where the
weights should be proportional to the number of
nonmissing entries in each data set [16].
''

`` 
Whenever more than one origin of information is
available, be it a single sensor or an ensemble of
observations, conflicts, contradictions, and inconsistencies
may occur. If data are fused at the decision level, then a
decision or voting [8] rule may be applied, as in the fusion
of different classification maps in remote sensing (see
Example II-C.1). Other approaches, related to multisensor
data fusion, are discussed in [9] and [157]. When only two
data sets are confronted, more elaborate solutions may be
required. An obvious challenge is to devise a suitable
compromise. A more fundamental challenge, however, is
identifying these inconsistencies.
''


\cite{butler2018alignmentscore}

``
"We calculated an alignment score as follows. First, we randomly downsample the datasets to have the same number of cells as the smallest dataset. Then, we construct a nearest-neighbor graph based on the cells’ embedding in some low dimensional space (the aligned CC space after running the alignment procedure). For every cell, we then calculate how many of its k nearest-neighbors belong to the same dataset and average this over all cells to obtain x¯. If the datasets are well-aligned, we would expect that each cells’ nearest neighbors would be evenly shared across all datasets. For all of our examples, we chose k to be 1\% of the total number of cells. We then normalize by the expected number of same dataset cells and scale to range from 0 to 1.")
''

\[\text { Alignment Score }=1-\frac{\bar{x}-\frac{k}{N}}{k-\frac{k}{N}}\]



\cite{Kuchroo2021integrated-diffusion}

``
Recently, alternating diffusion has been proposed to combine diffusion operators created from multimodal data~\cite{katz2019alternating-diffusion}. Intuitively, this generalizes the random walk to “hop” between different metric spaces by taking a matrix product of the Markov transition matrices $P(xi,xj) = PiPj$ (5) Finally, the resultant alternating diffusion operator P is powered to stimulate “hopping” across modalities. While this approach is able to construct a joint diffusion operator, it is sensitive to local and global noise found in each dataset creating a joint manifold that represents not only modality specific sources of information, but also noise.
''

``
Each of these datasets contains nonoverlapping features with different scales, and is subject to differing degrees of noise. Here, we propose an approach for generating an integrated diffusion operator that selects information from both modalities at multiple scales.

Our approach is based on the idea that frequency components of the diffusion operator can be low-pass filtered using particular powers of this operators. By using multiple scales, we perform both local and global denoising of the data modalities to a degree where highly relevant information is retained in the joint integrated operator. This integrated diffusion operator can then be used to visualize and denoise both datasets
''

``
Powering directly by t1, t2 and tintegrated would lead to an oversmoothing effect that would eliminate information from the low frequency eigenvectors in the final computed manifold, effectively collapsing independent informative data points together. To alleviate this concern, we raise each modalities diffusion operator to the lowest possible multiple of the ideal view-specific t. This means we can write our integrated diffusion operator, J, to reflect the differing levels of global information between views as $J =P_1^{t_1} 1P_1^{t2_}$
''


\cite{Ham2003LearningHD} (Use PCA, FA, and LLE to attempt to reconstruct the second domain using constrained optimization)
``
Suppose, however, that the desired outputs are not discrete labels, but are themselves high dimensional examples from another data set. In such a problem, the goal is not to classify the inputs, but to learn their high dimensional correspondences. One solution to this problem is to learn common low dimensional representations for different high dimensionaldata sets. Dimensionality reduction has been extensively studied in the framework unsupervised learning, but not generally with the idea of putting high dimensional examples from different data sets into correspondence. For these reasons, the problem of learning high dimensional correspondences is best tackled by a mixture of supervised and unsupervised methods.
''

``
One popular approach in unsupervised learning is to model the data as lying on a linear subspace embedded in a high-dimensional space. The projections of the data along the bases of the linear subspace then constitute a low-dimensional representation of the data. In the context of the correspondence problem, this low-dimensional representation should be consistent between the two different data sets. By treating the correspondence problem as a large missing data problem, it is possible to simultaneously learn a consistent low-dimensional representation as well as fill in the unknown high-dimensional missing values. In order to handle this missing data problem, we consider these algorithms within a generative model framework.
''

``
Intuitively, this causes the two different manifold structures to align with each other to bring these common points into correspondence. This is illustrated on some simulated data in Figure 3 where two different manifolds were sampled to generate the datasets X and Y. Due to the low sampling density, LLE applied separately to the datasets gives rise to a non-faithful representation. However, constraining equivalent points in the two datasets to have the same underlying two-dimensional representation causes the underlying uniform manifold structure to become apparent.
''

``
In order to reconstruct the unknown correspondence of an example in dataset X, the low-dimensional representation in Y is first computed. Then, by finding the nearest points in X to this representation, the corresponding image is reconstructed by interpolating the appropriate examples in X.
''

\cite{wang2011hetero-domain-adapt}
``
...the availability of a large amount of labeled data to train a model. However, labeled data is often expensive to obtain. To save labeling effort, in many situations we want to transfer labeled information from one domain to another. This problem arises in a variety of applications in information retrieval, e-commerce, computer vision, and many other fields. To address this problem, the area of transfer learning in general, and domain adaptation in particular, has recently seen a surge of activity ... However, one limitation that has not been fully addressed is that most existing domain adaptation approaches assume that the source and target domains are defined by the same features, and the difference between domains primarily arises due to the difference between data distributions. This assumption is not valid in many scenarios such as cross-lingual retrieval and multimodal datasets involving words and images, where the source and target domains do not share common features.
''

[APPROACH] - Use of labeled information: the authors form three separate kernel-like matrices: two are binary 1-0 matrices defining either similarity or dissimilarity, the third is constructed from a gaussian kernel. The optimization problem (minimizing similarities, maximizing differences) seeks a common topological space combining all three kernel matrices.
`` 
We treat each input domain as a manifold. The goal is to construct K mapping functions to project the input domains to a new latent space preserving the topology of each domain, matching instances with the same labels and separating instances with different labels. To achieve this goal, we first create a matrix representation of the joint manifold modeling the union of all input domains. Each manifold is represented by aLaplacian matrix constructed from a graph defined by an “affinity” measure connecting nearby instances. The label information plays a key role in joining these adjacency graphs, forcing the instances with the same labels to be neighborsand separating instances with different labels. The joint manifold has features from all input domains, so its feature space is redundant. To remove the redundant features, we project the joint manifold to a lower dimensional space preserving manifold topology. T
''


\cite{shen2017manifold-matching}

APPROACH: The pairwise distances between within each domain are normalized. Only the distances < threshold (k) are kept within each row. Within each domain, the shortest path distances are calculated. Each domain is then mapped to d dimensions via MDS. Procrustese analysis is finally used to align the two manifolds. NOTE: Training data must be corresponded and of the same size!

NOTE: View discussion section about extending to test points.
``
 A naïve procedure is to pick one nonlinear algorithm, apply it to each modality separately, and match the embedded modalities. But such a simplistic procedure does not always guarantee a good matching performance, since many non- linear embedding algorithms only preserve the local geometry up to some affine transformation [13] . Furthermore, using nonlinear transformations separately can even deteriorate the matching per- formance when compared to using simple linear transformations, as shown in our numerical simulations. 
''

``
 Ideally, a good matching procedure should be able to correctly identify the corre- spondence of the new observations, i.e., if the testing observations are truly matched in the context, the mapped points should be very close to each other in R d . If the testing observations are not matched, the mapped points should be far away from each other. 
''

``
 To estimate the testing power for given data, we first split all observations into matched training data pairs, matched testing data pairs, and unmatched testing data pairs. After learning ρl from the matched training data and applying them to all testing data, the test statistic under the null hypothesis can be estimated from the matched testing pairs, and the test statistic under the alternative hypothesis can be estimated from the unmatched testing pairs. The testing power at any type 1 error level is directly estimated from the empirical distributions of the test statistic, and a higher testing power indicates a better manifold matching algorithm. 
''

``
Note that MMSJ merely requires the training observations from different modalities to be corresponded and of same size, but the testing observations from different modalities can be of different and arbitrary size, because they are separately mapped within each modality and of unknown correspondence. In the numerical experiments we opt to set the testing data to be of the same size for convenience of presentation and evaluation.
''

``
MMSJ starts with two distance matrices rather than the sample observations directly, which means it is directly applicable to multiple modalities of different feature dimensions, as long as a distance metric can be defined for each modality. Although there is no limitation on applying the algorithm once the distances are given, the actual matching performance is clearly dependent on the choice of the metric. 
''

``
Using the joint neighborhood graph allows the resulting shortest-path distance to utilize the dependency structure of the training data. Computationally, the shortest-path distance matrix can be effectively implemented by Floyd’s algorithm or Dijkstra’s algorithm [43] , which can be further sped up by choosing a small set of landmark points [3,38] . Theoretically, the shortest-path distance can recover the geodesic distance of isometric manifolds with high probability under certain sampling conditions [4,38] . When embedding the testing data, we essentially treat the train- ing data as landmark points and only compute the shortest-path distances from the testing data to the training data. 
''

``
For the testing data, they are embedded by out-of-sample MDS, which is a standard technique for MDS and kernel PCA [3,32,46] and more efficient than re-embedding all training and testing data. After all testing data are mapped onto the manifolds by the learned Procrustes matching, 
''


\cite{keselman2003many-graph-matching}

The authors of \cite{} use a many-to-many graph matching approach based on shortest path distance (using Earth-Mover's Distance). They first project the two domains in to a normed space via PCA. Their many-to-many approach is not limited to one-to-one correspondance.


\cite{gori2005graph-matching-rw}

`` (Speaking of their approach based on PageRank):
. Interestingly, we show that
the proposed approach is not only appropriate for graph
isomorphism, but that it is also very well-suited for dealing
with partial and approximate graph matching derived for
instance from problems of image retrieval. The objects of the
visual collection that we consider are properly represented
by graphs, whose node’s labels contain visual features. The
retrieval is based on partial matching of graphs in a way
that closely reminds us the proposed approach to graph
isomorphism. 
''

\cite{bai2004graph-matching-specral}
``
In this paper we investigate whether methods from manifold learning theory can be combined with spectral graph
theory to develop effective tools for graph structure matching. The idea is to use manifold learning methods to embed the graphs in a low dimensional coordinate space, and
to perform spectral analysis on the co-ordinate data for the
embedded graph-nodes. We proceed as follows. We commence by using a strategy similar to ISOMAP [7] to embed
the graphs in a Euclidean pattern space. This is done by
computing a matrix of shortest(geodesic) distance between
nodes in the graph. We then apply MDS (Multidimensional
Scaling) [16] to the distance matrix, and this embeds the
individual nodes of the graph in a Euclidean space. Once
embedded in this space, we can apply a variant of the Scott
and Longuet-Higgins [4] algorithm to match the two sets of
embedded points. By doing this we overcome problems of
structural difference.
''


\cite{kim2017discoGAN}
DiscoGAN - Similar to MAGAN, but with no explicit pairing. Used to match handbags and shoes, align objects, and to match up faces.




\cite{wang2008ma-procrustes}
``
Manifold alignment is very useful in a variety of applications since it provides knowledge transfer between two seemingly disparate data sets. Sample applications include automatic machine translation, representation and control transfer between different Markov decision processes (MDPs), image comparison, and bioinformatics.
''














%To a given point $x_i$, the nearest anchor within the domain $\mathcal{X}$ may not correspond to the nearest anchor of the true correspondence to $x_i$ in domain $\mathcal{Y}$, provided a true correspondence exists. That is, even if $x_i$ corresponds to $y_j$, $a_{x_i}$ does not necessarily correspond to $a_{y_j}$.



 % First, we determine the shortest path from $x_i$ to each anchoring point within $\mathcal{X}$. The shortest of these determines the nearest anchor to $x_i$, or $a_{x_i}$. Next, the shortest path between this anchors correspondence in $\mathcal{Y}$ and $y_j$ is determined. From the other direction, we can determine the shortest distance from $y_j$ to its nearest anchor in $\mathcal{Y}$. 

 % From here, we calculate the distance from the anchor's correspondence in $\mathcal{X}$ to $x_i$. The nearest anchor to $x_i$ may not correspond to the nearest anchor to $y_j$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 % $\Tilde{d}(x_i, x_j) = \frac{d(x_i, x_j)}{\max(\mathcal{D}_{\mathcal{X}})}$, where $\mathcal{D}_{\mathcal{X}}$ is the set of all pairwise distances in set $\mathcal{X}$.
